Repeating Work Can Lower Energy per Successful Goal in LLM Agents

When a temporary call failure interrupts a tool-using LLM agent, the framework must choose how much completed work to repeat. Repeating less completed work intuitively saves computation, but recovery mechanisms also change subsequent execution and the chance of success. We compare recovery mechanisms by energy per successful goal (EpG), which divides the energy of all task runs (including failed runs) by the number that finish correctly. In controlled vLLM experiments on one node, we measure board energy above idle for eight recovery options on reliably solved multi-turn tasks, with selected comparisons across three model families. For the model tested across all eight options, with the prefix cache retained, starting over has 22 percent lower EpG than continuing after early failures. Under the same cache condition, continuing has 24 percent lower EpG than starting over after late failures. Among all eight recovery options, repeating only the interrupted turn has the lowest observed EpG after early and late tool failures on this model. Holding recovery fixed, retaining the prefix cache reduces prompt tokens needing fresh computation by 86 percent but reduces recovery energy by only 8 percent at contexts up to 7,333 tokens. These measurements and a condition relating recovery energy and success show when repeating work lowers EpG, helping framework developers choose how their agents recover on their intended models and tasks.

==> tables/m23_table_clean.tex <==
\multicolumn{8}{l}{\textit{Mistral Small 3.2 24B}} \\
Malformed & early & 8/8 & \textbf{4{,}887} & 6/8 & 6{,}785 & 7/8 & 5{,}735 \\
Rate limit & early & 7/8 & \textbf{5{,}078} & 6/8 & 5{,}812 & 6/8 & 6{,}216 \\
Tool error & early & 8/8 & 4{,}984 & 7/8 & \textbf{4{,}717} & 7/8 & 5{,}380 \\
Timeout & early & 8/8 & 5{,}038 & 7/8 & \textbf{4{,}775} & 7/8 & 5{,}531 \\
Malformed & late & 8/8 & 7{,}144 & 8/8 & \textbf{4{,}330} & 7/8 & 5{,}201 \\
Rate limit & late & 8/8 & 6{,}912 & 6/8 & 6{,}244 & 7/8 & \textbf{5{,}026} \\
Tool error & late & 8/8 & 7{,}013 & 7/8 & \textbf{4{,}990} & 7/8 & 5{,}323 \\
Timeout & late & 7/8 & 7{,}921 & 7/8 & \textbf{4{,}660} & 7/8 & 5{,}311 \\
\midrule
\multicolumn{8}{l}{\textit{gpt-oss 20B}} \\
Malformed & early & 11/12 & 2{,}848 & 6/12 & 5{,}648 & 11/12 & \textbf{2{,}842} \\
Rate limit & early & 10/12 & \textbf{2{,}725} & 8/12 & 3{,}974 & 9/12 & 4{,}970 \\
Tool error & early & 12/12 & \textbf{2{,}428} & 9/12 & 3{,}781 & 8/12 & 3{,}960 \\
Timeout & early & 10/12 & \textbf{3{,}690} & 6/12 & 5{,}453 & 9/12 & 4{,}158 \\
Malformed & late & 10/12 & 5{,}307 & 11/12 & \textbf{2{,}559} & 9/12 & 3{,}581 \\
Rate limit & late & 12/12 & 3{,}410 & 10/12 & 2{,}666 & 11/12 & \textbf{2{,}564} \\
Tool error & late & 11/12 & 3{,}701 & 12/12 & \textbf{2{,}226} & 10/12 & 3{,}856 \\
Timeout & late & 10/12 & 5{,}336 & 11/12 & \textbf{2{,}409} & 11/12 & 2{,}867 \\
\bottomrule

